An SR Flip-Flop based Physical Unclonable Functions for Hardware Security

Physical Unclonable Functions (PUFs) have emerged as a promising solution to identify and authenticate Integrated Circuits (ICs). In this paper, we propose a novel NAND-based Set-Reset (SR) Flip-flop (FF) PUF design for security enclosures of the area- and power-constrained Internet-of-Things (IoT) edge node. Such SR-FF based PUF is constructed during a unique race condition that is (normally) avoided due to inconsistency. We have shown, when both inputs (S and R) are logic high ('1') and followed by logic zero ('0'), the outputs Q and Qbar can settle down to either 0 or 1 or vice-versa depending on statistical delay variations in cross-coupled paths. We incorporate the process variations during SPICE-level simulations to leverage the capability of SR-FF in generating the unique identifier of an IC. Experimental results for 90nm, 45nm, and 32nm process nodes show the robustness of SR-FF PUF responses in terms of uniqueness, randomness, uniformity, and bit(s) biases. Furthermore, we perform physical synthesis to evaluate the applicability of SR FF PUF on five designs from OpenCores in three design corners. The estimated overhead for power, timing, and area in three design corners are negligible.

==> 5_conclude.tex <==
\section{Conclusion}
\label{sec:conclusion}

In this work, we have proposed to use the existing SR flip-flop in the design to quantify its race condition for PUF implementation. We embed a centroid architecture with SR FFs so that PUF responses conform to local transistor variations only. The generated responses exhibit better uniqueness, randomness, reliability and reduced bit-aliasing compared to other metastability-based PUFs. For future work, we would evaluate the uniqueness of SR-FF PUF responses from transient noise based simulation and  the resilience  against adversarial machine learning attack.



% In this work, we have proposed a new PUF architecture using the existing SR flip-flop in the design to quantify its race condition using SPICE simulations. We reuse the existing SR-FF in a design with a centroid architecture so that PUF responses conform to local transistor variations only. The responses also exhibit better uniqueness, randomness, reliability and reduced bit-aliasing compared to other metastability-based PUF. For future work, we would evaluate the uniqueness of SR-FF PUF responses from transient noise based simulation and  the resilience  against adversarial machine learning attack.

%under accelerated aging testing and scalability for true random number generation in reconfigurable platform. 




==> 6_miscel.tex <==
% \section{Miscellaneous}
% \textit{Motivation/Why do we care about this problem and the results?}
% \begin{itemize}
% \item Importance of the work and its impact
% \item Difficulty of the work
% \item Impact it has if successful/ broader implication 
% \end{itemize}


% \textit{Problem statement}
% \begin{itemize}
% \item Problem we are trying to solve (should show interesting and innovative ideas that contribute to the field)
% \item Scope of the work
% \end{itemize}

% \textit{Approach}
% \begin{itemize}
% \item How did you solve the problem?
% \item Did you use the simulations, analytical models, made a prototype or used field data?
% \item What important variables did you control,ignore  or measure?
% \end{itemize}

% \textit{Results}
% \begin{itemize}
% \item What happened in the experiments?
% \item What are the major results of the experiment?
% \end{itemize}


% \textit{Conclusions}
% \begin{itemize}
% \item Implications of the answer
% \item Generalized result or specific to a case?
% \item Why do you believe this paper has impact?
% \end{itemize}

==> google_doc_resullt.tex <==
https://docs.google.com/a/mail.usf.edu/spreadsheets/d/1Sxt4rZj0u7o6DwE7hjeqZbqryzpaGuebdV-_15hav-Y/edit?usp=sharing

==> review.tex <==

--------------------------------   HOST 2019 review -------------------------------


----------------------- REVIEW 1 ---------------------

----------- Overall evaluation -----------
1/ The authors describe how previous publications (for many different reasons) require large area and this is the main motivation and their circuit reuse is supposed to reduce this cost. As I detail below, I believe the "reuse" claims in this manuscript are far from solid and will require a more substantial proof. also the actual cost is not well covered. I relate to this point in more detail in comment 2.

2/ REUSE claims are not sufficiently solid: trying to use the same FF in a design for both purposes is a bit too much at this stage of a simulation based work from several reasons:
a) you need to build a standard-cell for achieving good/ long enough metastable state -->design is fully custom or hard and require cell characterization and design.
b) The designed cells will suffer in performance and area in normal mode significantly because they are not optimized for robustness and speed etc. --> you clearly did not relate to these cost (overhead) factors in analyzing overheads.

3/ I think that this work lacks a far more detailed examination of local /inter-die and intra-mismatch variations analysis on this circuit while changing design parameters (devices length wire length etc.). This is of coarse to better understand the effects, trade-offs and mechanisms, the (circuit and physical) analysis here is quite short and lack evidence. 

4/ Relating to the previous comment. For example, once the device in a metastable state, the "randomness" of the results really depends on many factors which are not covered here and depend on physical parameters: the inter-transistor routings, inter-gate routings, aggressive supply voltage changes (adversary), pulse-width of the SR signal where the mechanism to generate it also depends on variations etc. and was not covered in this work. The device "balancing" parameters and optimization of the output NAND to "linger" on VDD/2 and not on a "very-biased" value is not covered.

5/ For me these results are quite "theoretic" for a work which is "physical" (especially for PUFs which rely on physical phenomena):  Designs are IDEAL with no layout / routing and parasitic capacitances values in simulation --> this is far from reality and put in doubt many aspects. In practice, due to layout sensitivities you might find out that the total area cost at the end will be substantial and you will also perhaps need replica circuits, majority etc. And even if you do not have silicon or implementation you should at least perform Layout base examination.

7/ I found it strange that as part of the UNIQUENESS examination of the responses you did not perform a noise-simulation based analysis --> today it is possible to perform transient noise simulation to verify that the PUF response is solid even in noisy environment (especially if it is mixed with the high-activity logic ...). Another consideration is to make sure the adversary cannot further tamper with the device / noise-level etc. to bias the responses. 

8/ results presentation --> In my opinion either you:
a) overlay histograms one on the other
b) summarize mean and variance values in a table.
c) summarize the values in a condensed Figure.
This is because the results are presented is a quite exhausting and repeating way and it looks more like a report in this sense. I believe the authors can present the results in a more compact and intuitive fashion.


----------------------- REVIEW 2 ---------------------

----------- Overall evaluation -----------
A NAND-based Set-Reset (SR) FF PUF design is proposed in which both S and R are driven from 1 to 0, creating a race condition. SPICE simulations are used to investigate the SR FF PUF in 90, 45 and 32 nm technologies. An SR-FF PUF is proposed that builds on the SR FF PUF proposed previously, e.g., reference [9]. The authors describe their contribution as developing a version that does not require ECC or helper data.

The authors discuss inter-chip variations as contributing to uniqueness and intra-chip variations `determines the reliability of the key'. These attributions are not generally accepted by the community. Inter-chip variations are difficult to leverage because of the limited range of chip-to-chip variations and the corresponding decrease in uniqueness in the bitstrings as the population grows. Intra-chip variations are generally accepted as the best source of variations for uniqueness and randomness, and is not related to reliability as claimed by the authors.

The description in Section III, starting with the 3rd paragraph is not well written. This sentence is difficult to interpret: "If the next set of input signals (M2-M3 and M6-M7) being low) appear within the active edge of CLK before receiving any handshaking signal (e.g., data valid), non-binary values would appear in both OUT3 and OUT4". What does it mean to have non-binary values? Also, how would you `vary transistor length or threshold voltage of one of the output NAND gate to increase the delay variability"?

Results in Section IV.A are difficult to interpret. The authors state "It has been shown that the average HD for different key-length except 128-bit is close to 49\%". This does not appear to be the case for the data in Fig. 5.

Later, the authors show that reliability is > 90\% and then state "If we discard 10\% responses where HD > 0, we can achieve reliability of 100\%". How would this be done in practice? This is not convincing evidence to support a PUF without ECC or helper data.


----------------------- REVIEW 3 ---------------------

----------- Overall evaluation -----------
At the beginning, an introduction to PUFs is given.
They authors claim to have a novel design of an SR FF based PUF, which is also analyzed/benchmarked 
in the paper.  
After this, background knowledge and related work is given, followed by the introduction of the
proposed cross-coupled SR Flip Flop.
Furthermore, Spice simulations and results are illustrated and at the end a conclusion is given.

- The paper is written in a clear and understandable English.
- The benchmarking is not completely done with the systematic method claimed in the paper. See:
  Maiti, Abhranil, Vikash Gunreddy, and Patrick Schaumont. 
  "A Systematic Method to Evaluate and Compare the Performance of Physical Unclonable Functions."
  Embedded systems design with FPGAs. Springer, New York, NY, 2013. 245-267.
- Why is the inter-chip HD for 64- and 128-bit key nearly the same?
- All in all this paper needs major rework in order to provide a solid contribution to PUF research.

Misc.:
- Abbreviations should appear again after the abstract.
- Same X-axis scaling of same Bit width makes it easier to compare plots.
- To much figures for the measurement, makes it difficult to understand the paper.
  Perhaps the core statements should be summarized in table a table.


----------------------- REVIEW 4 ---------------------

----------- Overall evaluation -----------
This paper proposes a Set-Reset (SR) Flip-flop (FF) PUF design. The design is based on NAND gate and utilizes the inconsistency of path delay on outputs of SR-FF. When the value of inputs S and R are set to '1' and followed by '0', then the value of outputs Q and Q-bar will be inconsistent depending on statistical delay variations. The architecture of the proposed PUF design has multiple parallel SR-FF and the CRP is generated from all these SR-FFs. The paper provides simulation analysis of uniqueness, reliability, and uniformity.

According to the result from hspice simulation, the proposed PUF design shows a very good performance on uniqueness, randomness, and reliability.


Reviewer Suggestions / Weakness:

1) The SR FF with the use of 1 and 0 on SR are equal to D-FF. The paper does not discuss how this proposed design is novel.
2) There is no real experiment in this work. The result comes from hspice simulation. However, since PUF is a hardware-based design, the software-based simulation cannot be considered to describe process variation.

==> todo.tex <==


